Towards Practical Capture of High-Fidelity Relightable Avatars

In this paper, we propose a novel framework, Tracking-free Relightable Avatar (TRAvatar), for capturing and reconstructing high-fidelity 3D avatars. Compared to previous methods, TRAvatar works in a more practical and efficient setting. Specifically, TRAvatar is trained with dynamic image sequences captured in a Light Stage under varying lighting conditions, enabling realistic relighting and real-time animation for avatars in diverse scenes. Additionally, TRAvatar allows for tracking-free avatar capture and obviates the need for accurate surface tracking under varying illumination conditions. Our contributions are two-fold: First, we propose a novel network architecture that explicitly builds on and ensures the satisfaction of the linear nature of lighting. Trained on simple group light captures, TRAvatar can predict the appearance in real-time with a single forward pass, achieving high-quality relighting effects under illuminations of arbitrary environment maps. Second, we jointly optimize the facial geometry and relightable appearance from scratch based on image sequences, where the tracking is implicitly learned. This tracking-free approach brings robustness for establishing temporal correspondences between frames under different lighting conditions. Extensive qualitative and quantitative experiments demonstrate that our framework achieves superior performance for photorealistic avatar animation and relighting.

==> figs/fig_ablation.tex <==
\begin{figure*}%[t]
    \centering
    \begin{minipage}[t]{\linewidth}
        \centering
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/light1_resize.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f3_nl_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f3_env_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f3_lcl_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f3_ts_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f3_ours_crop.png}
    \end{minipage}

    \begin{minipage}[t]{\linewidth}
        \centering
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/light2_resize.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f1_nl_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f1_env_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f1_lcl_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f1_ts_crop.png}
        \includegraphics[width=\onesixthfigurewidth\linewidth]{images/ablation/f1_ours_crop.png}
    \end{minipage}

    \vspace{5pt}
    \begin{minipage}{\linewidth}
        \centering
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{Light}
        \end{minipage}
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{NL}
        \end{minipage}
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{NL + ENV}
        \end{minipage}
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{NL + LCL}
        \end{minipage}
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{NL + TS}
        \end{minipage}
        \begin{minipage}[t]{\onesixthfigurewidth\linewidth}
            \centering
            \subfloat{Ours}
        \end{minipage}
    \end{minipage}
    \caption{Ablation study results about our physically inspired linear light branch for the appearance decoder $\colordecoder$.
     The input environment maps are shown on the left.
    The relighting results of four alternative baseline approaches (see detailed explanations in Section 5.3 of the main text) and ours are shown on the right.
    }
\label{fig:ablation}
\end{figure*}


==> tables/tab_ablation.tex <==
\begin{table}
\center 
\caption{Quantitative evaluation results of ablation study. In each column, the best number is highlighted in \textbf{bold} and the second best one is shown with an \underline{underscore}.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccc|ccc}
\hline
           & \multicolumn{3}{c|}{Subject 1} & \multicolumn{3}{c}{Subject 2} \\ \hline
Method     & MAE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$  & MAE $\downarrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ \hline
NL        & \textbf{7.30}          & \underline{0.736}  & \underline{0.372}       & \textbf{6.38}         & \underline{0.746}   & \underline{0.368}      \\
NL + ENV & 16.93          & 0.691    & 0.393     & 13.01         & 0.684     & 0.398    \\
NL + LCL & 14.46          & 0.682    & 0.403     & 12.03         & 0.668     & 0.410    \\
NL + TS  & 11.42          & 0.695     & 0.385    & 9.71         & 0.703      & 0.381   \\
Ours       & \underline{7.34}          & \textbf{0.744}   & \textbf{0.307}      & \underline{6.54}         & \textbf{0.760}  & \textbf{0.314}       \\ \hline
\end{tabular}
\label{tab:ablation}%
}
\end{table}

